Efficient Dataframe Systems: Lazy Fat Pandas on a Diet

Pandas is widely used for data science applications, but users often run into problems when datasets are larger than memory. There are several frameworks based on lazy evaluation that handle large datasets, but the programs have to be rewritten to suit the framework, and the presence of multiple frameworks complicates the life of a programmer. In this paper we present a framework that allows programmers to code in plain Pandas; with just two lines of code changed by the user, our system optimizes the program using a combination of just-in-time static analysis, and runtime optimization based on a lazy dataframe wrapper framework. Moreover, our system allows the programmer to choose the backend. It works seamlessly with Pandas, Dask, and Modin, allowing the choice of the best-suited backend for an application based on factors such as data size. Performance results on a variety of programs show the benefits of our framework.

==> building_blocks.tex <==

\section{Building Blocks}
\label{sec:building:blocks}

In this section, we discuss the building blocks for our approach. 
\textcolor{red}{Do we really need this section? Redistribute to later sections?}

%Firstly, we discuss the data structures used by us. We discuss the control flow graph that represents various paths on which a program's execution may proceed to. Then we discuss data flow analysis (DFA) and live variable analysis (LVA). We also discuss Soot which is an optimization framework for java that we have extended for analysis of python code. We also discuss lazy vs eager evaluation and task graph analysis. 
%\subsection{Data Structures used}
%We briefly discuss the data structures used for the conceptualization and implementation of our approach:

\textbf{I don't see the word region being used anywhere later in the paper.  Why are we even mentioning it}
\paragraph{\textbf{Program Regions}}


% \begin{figure}[tbp]

% \centering
% \includegraphics[width=2.0in,height=3.0in]{figures/DAG.drawio.png}
% \caption{Task graph of Program in Figure ~\ref{fig:lfp_arch}}
% \label{fig:DAG1}
% \end{figure}



\paragraph{\textbf{Control Flow Graph and Data flow analysis}}
\label{dfa}
\label{lva_label}

%\subsubsection{\textbf{Control Flow Graph}}
%\label{cfg_label}

\textbf{We have two representations, region and CFG.  Need to explain why we need both, and if we construct one from the other}


\paragraph{\textbf{Live variable Analysis (LVA)}} 
\paragraph{\textbf{Soot}}



\paragraph{\textbf{Eager vs Lazy Evaluation}}


\paragraph{\textbf{Task Graph and Optimization}}
\label{TaskGraph}


% Program Analysis reasons about the behaviour of a program without actually running it. Optimizations based on task graph analysis are motivated from program analysis in this sense. However, they are different from program analysis in multiple ways:
% \begin{enumerate}
%     \item Program analysis is performed at compile time whereas task graph analysis is performed at execution time.
%     \item In program analysis, we traverse a control flow graph generated statically from a program whereas in task graph analysis, we traverse a task graph created from lazy execution of a program.
%     \item In program analysis, the whole program is analysed whereas in task graph analysis, only the task graph created for lazy API is analysed.
%     \item Program analysis requires detailed analysis of loops and conditions whereas in task graph analysis, loops are exploded and conditions are already executed. 
% \end{enumerate}

% Optimizations based on task graph analysis can improve the performance of an application by using a number of techniques like operation fusion, operation elimination, operation rearrangement, etc. We apply such techniques in the Section ~\ref{runopt} to perform run time optimizations in LaFP.

==> compile_opt.tex <==

\section{Compile Time Optimizations}
\label{comopt}
Many programs can be optimized by manually rewriting them using appropriate API features. However,  many users are not aware about these features. The availability of a number of different frameworks and their different APIs further complicates the problem. Our platform overcomes these challenges. We automatically perform these optimizations during the first phase of our optimization framework i.e JIT static analysis and optimization phase. We discuss a number of optimizations we have identified and implemented so far:  
\subsection{Data (Column) Selection}
\label{DS}
% Data Selection is performed to load only those data items into memory that are
% further used in the program. This optimization reduces memory footprints of a program. 
In many programs, all the columns (attributes) from the dataset are not used. Fetching such unused columns in the memory leads to memory wastage. Therefore, data (column) selection is performed to identify and to fetch only those used columns into memory. Used columns of different dataframes are identified by performing live attribute analysis (LAA) as discussed below. Once LAA is performed, the IR is modified to rewrite the program to fetch only these used columns into memory.  
 
 
 
 \textbf{Live Attribute Analysis (LAA):}
 \label{laa_label}
LAA is an extension of live variable analysis as discussed in Section ~\ref{lva_label}. LAA treats attributes (columns) of a dataframe as a variable. Similar to a variable, a dataframe column is live at a program point if there is a path to exit along which it may be used in the program. However, attributes are different from variables in the following aspects: 
\begin{enumerate}
    \item There is a hierarchical relationship between a dataframe and its attributes. If the whole datframe is used at a program point, all attributes of that dataframe become live.
    \item Similarly, all attributes of a dataframe are killed at the point of definition of a dataframe.
    \item If a dataframe is created from other dataframe, all attributes of child dataframe are transitively attributes of the parent dataframe.
\end{enumerate}

\inred{we have not defined basic block in CFG.  We probably should}
For each basic block $n$, the set 
Gen$_n$ contains dataframe attributes that are used in $n$,
and and Kill$_n$ contains dataframe attribute that are defined (i.e. assigned) in $n$, and thus ``kill'' all earlier definitions (assignments) to these attributes.  
Formally:


\begin{equation}
  Gen\textsubscript{n} = \left\{
                \begin{array}{ll}
                  d.i\| ~\textrm{  attribute i of dataframe d is used in basic} \\
                        \textrm{block n and that use is not preceded  by a }  \\
                        \textrm{definition of dataframe d in the basic block n.}\\
                  
                  \textrm{}\\
                  d.\tau\| ~\textrm{dataframe d is used fully in the basic block}\\
                          \textrm{n and that use is not preceded by a definition} \\
                           \textrm{of dataframe d in the basic block n.}
                \end{array}
              \right\}
\end{equation}



\begin{equation}
      Kill\textsubscript{n} = \left\{
                \begin{array}{ll}
                  
                  \textrm{d.}\tau \|~\textrm{dataframe d is defined in basic block n} \\
                  \textrm{}\\
                  \textrm{d.i} \| ~\textrm{attribute i of dataframe d is defined in }\\
                  \textrm{basic block n } \\
                  
                \end{array}
              \right\}
\end{equation}

We next define sets In$_n$ and Out$n$ which merge local information provided by Gen$_n$ and Kill$_n$, with information from sucessor nodes of $n$, to identify global liveness information.
\begin{equation}
Out\textsubscript{n} =  \Cup_{s \in succ(n)} \textit{In}\textsubscript{s}
\end{equation}

\begin{equation}
\textit{In}\textsubscript{n} =  Gen\textsubscript{n} \cup  \{ \textrm{Out} \textsubscript{n}- \textrm{Kill} \textsubscript{n}  \} 
\end{equation}
\par
 Once LAA is performed, liveness information is available for all columns of all dataframes. Then, the IR is modified to fetch only those columns that are live at the out of the program point where dataframe is created.



\begin{algorithm}[bt!]
\caption{Algorithm for Data Selection } 
\label{algo:data_selection}
\begin{algorithmic}
\Procedure{\textbf{Data\_Selection}}{}

\State src $\leftarrow$ Transform program to \SCIRPy
\State cFG $\leftarrow$ buildCFG(src) 
\State lAA$\leftarrow$ performLAA(cFG)
\State unitIterator $\leftarrow$ cFG.getUnitGraph().iterator()
%ForEach{$ unit \in \text{unitIterator} $} {
%\For {each $unit$ in $unitIterator$}{
\ForAll{$ unit \in unitIterator$}

		        unitType $\leftarrow$ getType(unit)
                \If{unitType $=$ AssignmentStatement}
                  
                        \If{ unit $=$ df creation stmt}
                        % \LineComment Get all live attributes
                        \State  liveAttrs $\leftarrow$ lAA.getFlowAfter(unit)
                        % \LineComment  Get df instantiated  in the unit
                        \State dfName$\leftarrow$ getDFName(unit)
                        % \LineComment Get all live attributes for this df 
                        \State dfAttrs $\leftarrow$ getDFLiveAttrs(liveAttrs,df)
                        \LineComment Create a list stmt with these attrs 
                        \State stmt $\leftarrow$ getListStmt(dfAttrs, "SO\_column")
                        \LineComment insert stmt in method's body
                        \State insertBeforeInMethod(stmt,unit)
                        \LineComment Update unit to fetch these attributes
                        \State updatePDCreationStmt(stmt, unit, "usecols")
                       
               \EndIf %if df creation
                %if assignment stmt
	\EndIf	   	
	\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[bt!]
\caption{Algorithm for Data Selection } 
\label{algo:data_selection}
\begin{algorithmic}
\Procedure{\textbf{Data\_Selection}}{}

\State Transform program to \SCIRPy
\State Build control flow graph 
\State Perform  Live Attribute Analysis (LAA)
\State Identify df\_creation\_units
\ForAll{$ unit \in df\_creation\_units $}
\State Get live df attributes using LAA
\State Update unit to fetch only these attributes
\EndFor

\State Transform \SCIRPy\  to optimized program
                       
\EndProcedure
\end{algorithmic}
\end{algorithm}
\par
Live attribute analysis is performed on the program in Figure ~\ref{fig:lfp_arch}. This program has only one defined dataframe i.e. df. Similar analysis is performed if there are more than one dataframes defined in a program. Gen and Kill for each node are defined. This information is used to compute In and Out values for each node. No attribute of the dataframe are live at the end of the dataframe. Since this node prints the full dataframe, whole df is live at the In of this node, which is represented by $\tau.df$. The dataflow values are computed for the remaining nodes using the equations mentioned above. The dataframe is killed at node 2, where the dataframe is getting created. The attributes live at Out of the node 2 are:'pickup\_datetime', 'passenger\_count' and 'fare\_amount'.
\par Therefore, though the data file contains 26 columns, only these 3 columns are used in the program.  This information is used to fetch only these columns by inserting a list statement with these columns as elements and then using this list to fetch only these columns using 'usecols' parameter in pandas API call while creating the dataframe. The optimized version of the program in Figure ~\ref{fig:lfp_arch} is shown in Listing 1. 

 \begin{lstlisting}[language=Python, caption=Optimized version of Program in Figure ~\ref{fig:lfp_arch}]
import pandas as pd
SO_columns = ["pickup_datetime","passenger_count","fare_amount"]
SO_d_d_t = ["pickup_datetime"]
SO_c_d_t = {"passenger_count":"int64","fare_amount":"float32"}
df = pd.read_csv("data.csv",usecols=SO_columns,parse_dates=SO_d_d_t,dtype=SO_c_d_t)
df = df[df.fare_amount > 0]
df["day"] = df.pickup_datetime.dt.dayofweek
df = df.groupby(["day"])["passenger_count"].sum()
print(df)

\end{lstlisting}
\subsection{\textbf{Dropped Columns}} 
\label{colremoval}
Users use drop() API to remove unwanted columns from dataframe. Fetching columns and then removing them leads to unnecessary data fetch and eviction. Therefore, such columns in a program that are not used anywhere except that they are explicitly dropped from Dataframe are identified using live attribute analysis and the program is modified to not fetch these columns. All dropped columns for respective Dataframes are identified. Each of these is checked for usage in the program using LAA analysis. Dropped columns that are not used in the program are not fetched.



        
\subsection{Metatdata Analysis}
Metadata provides relevant information about stored data in traditional database systems. However, such information is not available in Dataframe systems. Every time a dataset is used in a program, it is accessed afresh. Metadata information like the types of columns, size of row, the approximate number of rows in the dataset is not maintained. Further, in some cases, dtype (datatype) identified by pandas can be further refined. As pandas doesn't automatically identify category and date data types, developers manually force an appropriate dtype once dataframe is created using functions like astype(). Fetching multiple columns as category dtype rather than as  objects is more efficient and reduces memory requirements. Such metadata information, if available, can be used to fetch datasets efficiently. 
\par Therefore, metadata analysis is performed to maintain a metastore with this kind of information. This metastore is accessed everytime a dataset is used in a program. If the meta-data about the dataset is available in the metastore, it is retrieved. If meta-data is not available, the dataset is probed and metadata is generated and stored in metastore.  Information like  modified time,  column names and types, approximate size of each row, and approximate number of rows in the dataset is currently maintained in the metastore.

\par In order to safely derive the metadata information, the whole dataset should be parsed. However, this can be time consuming, especially for large datasets. To ensure correctness of metadata, entire dataset is traversed asynchronously. We randomly traverse the dataset when it is encountered for the first time. However, this is an optional optimization and the users can set the flag if they want to turn-off this aggressive metadata analysis. It should be noted that we have not considered the time taken asynchronously for meta data analysis when we benchmark our framework as it is an asynchronous activity.
% \par Optimizations discussed in this section are safe but may not be precise due to the unavailability of certain information during static analysis time. Therefore LaFP performs these optimizations during runtime and is discussed in the following section.




% \begin{algorithm}[bt!]
% \caption{Algorithm for Building Metastore } 
% \label{algo:data_selection}
% \begin{algorithmic}
% \Procedure{\textbf{Meta Data Analysis}}{}

% \LineComment Build Metastore
% \State file $\leftarrow$ get data file full path

% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

==> run_opt.tex <==


\section{Run-Time Optimizations}
\label{runopt}

\par Traditional database perform several optimizations when a query is submitted and execute it based on an efficient query plan performing only the necessary computation. Lazy frameworks such as Spark also optimize DAG before execution. 
\par Dask, which can be used by LaFP as one of the back-end executors, performs the following optimizations on the task graph:
\begin{itemize}
    \item Culling the task graph i.e. removing unnecessary computations from task graph.
    \item Inlining constants and functions to improve parallelism. 
    \item Fusing operations to ensure their execution using the same worker.
\end{itemize}

Similarly, the runtime module of LazyFatPandas (LaFP) exploits the opportunity of lazy computations to perform optimizations in the task graph (DAG) at run time. LaFP performs optimizations like Predicate push down (row selection), Redundant operations elimination, Lazy Print etc. Optimized task graph is then executed using the selected executor. It should be noted that if any scalable framework like Dask is used as back-end, it may perform its own optimization on the task graph optimized by LaFP. We discuss a few of these optimizations:  
% LaFP also uses look ahead capabilities using program analysis for lazy evaluation. 
% At the same time, many of these frameworks do not support complete Pandas API whereas LaFP aims to support Pandas API to the maximum extent possible. 
% The execution of a particular task may be more efficient using one particular framework depending on the task and datasets. Users can use any back-end engine for execution based on the experience. 


\subsection{Row Selection (Predicate Push Down)}
\label{chapter:row_selection}
\par Performing selection operation early in databases (Predicate Push Down) reduces the size of relation and therefore, reduces the computation to be performed during other operations like joins. In Dataframe systems, filter operations (row selection) reduce the size of Datafames. Therefore, we perform filter/row\_selection optimization by identifying the row\_selection operations in the program and moving them closer to the data source. 
\par However, row\_selection optimization in Dataframe systems is quite different and more complex as compared to those in traditional database systems. Assignment operators potentially redefining dataframes are interspersed in the program which is not the case in query optimization. Therefore, it is non-trivial task as moving filter operations arbitrarily can  modify the semantics of the program and impact its output. In order to overcome this limitation,  conflict points are defined and filter operations are not moved beyond these points to ensure that the program's semantics are not modified.
\newline
\textbf{Conflict Points:} 
% There are certain cases when a filter operation can not be moved beyond certain point(s). We refer to these as conflict point(s) for those respective operations. Moving them past these conflict points can potentially modify the program's outcome.
We define conflict point(s) for an operation as point(s) beyond which it can not be moved without potentially modifying the output of the program. We define the following conflicts that can occur in a program. Here, operator \textit{u} precedes operator \textit{v} in the original program \textit{(program start ... u - v ... program end)}.

\begin{itemize}

    \item $modAttributes(u) \cap  usedAttributes(v) \neq \phi$ ,
    \newline
    u is non row\_selection statement and v is a row\_selection statement.
    \item $usedAttributes(u) \cap   usedAttributes(v)  \neq \phi$, 
    \newline
    u is row\_selection statement with aggregate and v is a row\_selection statement.
    \item $v \in (merge,explode)$, v has an operator that modifies number of rows in the Dataframe.
    \item $v \in (read,write)$, v interacts with terminal.
    
\end{itemize}

\par modAttributes and usedAttributes are motivated from program analysis. modAttributes of a statement represents all the columns of a dataframe that are modified in the statement. usedAttributes represents columns of a dataframe that are used in the statement. Aggregates operations modify a Dataframe and filter operations are not moved beyond aggregate operations. Some operators like explode, and merge can affect the number of rows, acting like conflict points for all data filter operations. We also consider reading/writing statement from the terminal as conflict points.
\par Further, consider case as shown in Figure \ref{figure:row_selectino_example2}(a). Here we can move row selection past statement 1 as in (b),  as R1 is present in both paths after statement 1. However, in the instance of (c), we cannot move it post statement 1 as it is not present in the second path. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/row_selection_example2.png}
	\caption{Control Flow Conflicts for Row Selection}
	\label{figure:row_selectino_example2}
\end{figure}



\par Row selection algorithm  \ref{algo:row_selection} optimizes the task graph \textit{G} representing the root of the final computation. For each operator \textit{v} in post-dfs order, operator \textit{v} and operator \textit{u} are swapped only if they don't have any conflict, operator v is a row selection but not operator u, and operator v is present in all paths from operator u to the final computed value in G. 





\begin{algorithm}[bt!]
\caption{Row Selection Algorithm}
\label{algo:row_selection}
\begin{algorithmic}

\Procedure{\textbf{Row\_Selection}}{task\_graph \textbf{G}}
  \ForAll {node \textit{v} in post-dfs order of task graph G}
    
    \LineComment {Push down the row selection to earliest point possible}
    
    \State $u \gets $ Immediate preceding operation of v in task graph

    \LineComment {u preceeds v in task graph (program start...u-v...end)}
     \If { (v is a row\_selection statement) \\
        \quad\quad\quad\quad \textbf{and} (u is not a row\_selection statement) \\
        \quad\quad\quad\quad \textbf{and} (has\_swap\_conflict(u,v) is \textbf{False}) \\
        \quad\quad\quad\quad\textbf{and} (v is live at all program paths from u to end)}
        
       \State Remove v from all other paths from u to end
       \State Swap(u,v) and \textbf{continue}
    \EndIf
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[bt!]
\caption{Check swap conflicts for Row Selection}
\label{algo:has_swap_conflicts}
\begin{algorithmic}
\Procedure{\textbf{has\_swap\_conflicts}}{task\_graph \textbf{u},task\_graph \textbf{v}}
  \ForAll {node \textit{v} in post-dfs order of task graph G}
  
    \LineComment {u preceeds v in task graph (program start...u-v...end)}
    \If {(usedAttributes(v) $\cap$ modAttributes(u)  $\neq \phi)$ \\
    \quad\quad\quad\quad\textbf{OR} (operator(u) in [Operators affecting df shape]) \\
    \quad\quad\quad\quad\textbf{OR} (operator(u) in [Agg, Op requires complete pass of data])}
    \State \Return True
    \EndIf
    \State \Return False
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[bt!]
\caption{Check for Row Selection statement}
\label{algo:is_row_selection}
\begin{algorithmic}
\Procedure{\textbf{is\_row\_selection}}{task\_graph \textbf{u}}

\If {(operation(u) is 'get-item') \\
    \quad\quad\quad \textbf{and} (u has 1 child) \\ 
    \quad\quad\quad \textbf{and} (operator\_of(child\_of(u))) in $[>, >=, <= <, ==, !=, \&, |]$}

    \State \Return True
    \EndIf
    
    \State \Return False
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[bt!]
\caption{Check for any merge conflict during row\_selection}
\label{algo:check_merge_conflict}
\begin{algorithmic}
\Procedure{\textbf{has\_merge\_conflict}}{task\_graph \textbf{u}, task\_graph \textbf{v}}


    \LineComment {Both u and v are row\_selection statements}
        \LineComment {u preceeds v in task graph (program start...u-v...end)}
  \If {(any operators(v) is in [Agg, complete dataset op])}
    \State \Return True

    \LineComment {No conflicts. Can be merged together}
    \EndIf
  
  \State \Return False

\EndProcedure
\end{algorithmic}
\end{algorithm}

% \newpage

\begin{figure}[tbp]
	\centering
	\fbox{\includegraphics[width=0.8\linewidth]{figures/row_selection_example1.png}}
	\caption{Example for row\_selection and extended\_row\_selection}
	\label{figure:row_selectino_example1}
\end{figure}



\begin{algorithm}[bt!]
\caption{Extended row\_selection}
\label{algo:extended_row_selection}
\begin{algorithmic}
\Procedure{\textbf{Row\_selection\_extended}}{task\_graph \textbf{G}}

  \ForAll {(node \textit{v} in post-dfs order of task graph G)}


    \While {(True)}

    \State $u \gets $ Immediate preceding operation of v in task graph
    
    \LineComment {u preceeds v in task graph (program start...u-v...end)}

     \If { (v is a row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (u is not a row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (has\_swap\_conflict(u,v) is \textbf{False}) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (v is live at all program paths from u to  end)}
        
       \State Remove v from all other paths from u to  end
       \State Swap(u,v) and \textbf{continue}
    \EndIf
    \\
     \If { (v is a row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (u is not a row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (has\_swap\_conflict(u,v) is \textbf{True}) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (v is live at all program paths from u to  end)}
        
       \State Consider (u,v) as \textbf{compound\_row\_selection}  and \textbf{continue}

    \EndIf
    \\

     \If { (v is a compound\_row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (has\_swap\_conflict(u,v) is \textbf{False}) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} (v is live at all program paths from u to  end) \\
        \quad\quad\quad\quad\quad\quad\textbf{and} ( (u is not a row\_selection statement) \\ \quad\quad\quad\quad\quad\quad\textbf{OR} (has\_merge\_conflicts(u, get\_row\_selection\_of(v)) is \textbf{False}))}
        
        \State Swap(u,v) and \textbf{continue}
    \Else \If {(v is a compound\_row\_selection statement) \\
        \quad\quad\quad\quad\quad\quad\quad\textbf{and} (v is live at all program paths from u to  end)}
           \State Consider (u,v) as \textbf{compound\_row\_selection} and \textbf{continue}
    
    \EndIf
    \EndIf


    \EndWhile
    \EndFor

\EndProcedure
\end{algorithmic}
\end{algorithm}





\subsection{Extended Row Selection Algorithm}
\par As discussed, row\_selection operations can not be moved beyond their conflict points. in order to overcome this limitation and further optimize the task graph, both operations i.e. the row selection along with its conflict points are considered as a single \textbf{compound\_row\_selection} operation which can be moved near to dataset fetching operation. Algorithm ~\ref{algo:extended_row_selection} shows idea of extended row selection to move row selection along with
their conflict points which are implemented partially.

\par Consider an example shown in Figure \ref{figure:row_selectino_example1}(a). Nodes in green represent row selection statements, and red nodes represent conflict statements. As seen in (b), R1 will be moved close to its conflict point. Similarly, in (c), R2 will be moved closer to its conflict point. If statement 1 and statement 2 do not conflict, then we can consider both R2 and statement 2 as a single compound row selection statement and move it past statement 1, as shown in (d). Since now, any code movement is not possible. We can merge R1 and R2 if there are no conflicts between them, as shown in (e).

\par By carefully observing the above two optimizations, we notice that we have intentionally omitted a case when there are two or more row selection statements together. We could merge them into a single row selection statement in this case. However, doing so will restrict other opportunities for moving individual statements. Therefore we perform this merging after no more row selection statement movement is possible.


\subsection{Redundant Operation Elimination}
\label{chapter:dead_code_remove}
Even small computations may take significant amount of time for execution when working on very large datasets. The resources deployed for computations are unnecessarily wasted if the results of the computations are not used in the program. Such computations are redundant and can be safely removed from the task graph without affecting the actual program output.


\par By representing the program as a task graph and invoking compute, we can remove unnecessary computations related to other data frames. However, in some cases, the computation performed within that dataframe, like adding/updating a column, may not be necessary to compute the final result. 



i	
\begin{figure}[htbp]
	\centering
	\fbox{\includegraphics[width=0.62\linewidth]{figures/redundant.png}}
	\caption{Condensed task graph with redundant operations}
	\label{figure:redundant_operation}
\end{figure}


Consider Figure \ref{figure:redundant_operation}, a condensed high-level task graph of Listing \ref{lst:dead_code_example}. Here, node(s) in red are not part of the final computation of Line 14 and will be automatically removed. Node(s) in yellow are updating intermediate results on which final computation is performed. However, they are redundant operations as they are not affecting/used in the final computation and could be safely removed. Node(s) in green is the final operations that should be executed.
%, and corresponding code is shown in Listing \ref{lst:dead_code_example_optimized}

% \newpage
\noindent
% \begin{minipage}{\linewidth}
    
	\begin{lstlisting}[language=python,label={lst:dead_code_example},caption={Example of redundant operation}]
import lazyfatpandas.pandas as pd
if __name__ == '__main__':
   df = pd.read_csv('data/yellow_tripdata_2015-01.csv')
   df['day'] = df.tpep_pickup_datetime.dt.dayofweek # add features
   df['discount'] = df.extra < 0
   df['taken_highway'] = df.tolls_amount > 0
   df = df[(df.fare_amount > 0) & (df.tip_amount > 0) \& (df.trip_distance <= 300)] 
   # Get valid tipped trips
   airport_trips = df[df.airport_fee > 0]
   long_distance = df[(df.fare_amount > df.fare_amount.max()*0.1)]
   total_refund = (long_distance.improvement_surcharge * long_distance.fare_amount + long_distance.tolls_amount).sum()

   print(total_refund.compute())
	\end{lstlisting}
% \end{minipage}


% \noindent
% \begin{minipage}{\linewidth}
% 	\begin{lstlisting}[language=python,label={lst:dead_code_example_optimized},caption={Optmized version of Listing \ref{lst:dead_code_example} after redundant operation}]
% import lazyfatpandas.pandas as pd
% if __name__ == '__main__':
%    df = pd.read_csv('data/yellow_tripdata_2015-01.csv', parse_dates=['tpep_pickup_datetime', 'tpep_dropoff_datetime'])
%    df = df[(df.fare_amount > 0) & (df.tip_amount > 0) \& (df.trip_distance <= 300)] 
   
%    long_distance = df[(df.fare_amount > df.fare_amount.max()*0.1)]
%    total_refund = (long_distance.improvement_surcharge * long_distance.fare_amount + long_distance.tolls_amount).sum()

%    print(total_refund.compute())
% 	\end{lstlisting}
% \end{minipage}

\par This algorithm is inspired by a static "\textit{strong liveness analysis}" \cite{618_program_analysis} technique. The following algorithm \ref{algo:remove_dead_code} is recursive and takes a task graph \textit{G} as input where the root represents the computation to be performed. It also takes two more parameters, one \textit{liveset}, representing columns used from that point until the final computation. Second, \textit{is\_start}, a boolean value represents whether it is a terminal node (final computation node) or not.


\par\noindent There are, in general, five cases that can occur.

\begin{itemize}
    \item The node is a \textit{compute()} type; then, we must evaluate all its sources as they represent different computations individually.
    
    \item The node is a start node (final computation node), then "liveset = usedAttributes" of the node, and this node will always be useful as it is the requested computation by the user.
    
    \item The node is a read operation, then it is useful only when there is at least one column live at that point that is read. In other words, some column from that source is used in later computations.

    \item The node is updating the dataframe, then the usedAttributes of the node becomes live only when the updated column is live. Also, if the node updates only the metadata like rename, then its modAttributes becomes live only when its usedAttributes is used in later computations.
    
    \item The node is reading the dataframe; its usedAttributes becomes live only when there are some common columns between the liveset and nodes' usedAttributes.

\end{itemize}


The task graph is modified with nodes marked as useful if they are used for computation. Therefore, non-useful nodes can be removed from the task graph and are not executed as they represent redundant operations.
\subsection{Lazy Print}\label{sec:lazy_printing}
DataFrame computations are deferred until the \texttt{compute} method is called. Frequent invocation of \texttt{compute} can be costly, as it requires optimizing the task graph and performing the actual computations.
While invoking compute for output statements like print is an option, frequent print statements forcing computation degrades the performance. To address this, we propose lazy printing, where print statements are executed lazily allowing multiple DataFrame computations to be aggregated and benefit from optimizations on larger task graphs.

\vspace{.15cm}

One approach to delay prints is to move print statements to the end of the program during JIT static analysis phase and use a temporary variable to hold the data needed for printing. However, this method is complicated and require frequent changes in source code. To minimize code changes, we leverage the runtime to delay print statements. This is achieved by treating print method call as an operation on the DataFrame and adding a corresponding node to the task graph like any other DataFrame based operation. When the task graph is executed, the print nodes are processed, and the data is printed.

\vspace{.15cm}

% \begin{mypython}[caption={Program with multiple print statements}, label=lazy_print_ex]
\begin{lstlisting}[language=Python, caption=Program with multiple print statements, label=lazy_print_ex]
import lazyfatpandas.pandas as pd
#Override  built-in print method with lazy print
print = pd.lazyPrint
df = pd.read_csv("data.csv", parse_dates=["pickup_datetime"])
print(df.head())  # lazy print
df["day"] = df.pickup_datetime.dt.dayofweek
passengers_per_day = df.groupby(["day"])["passenger_count"].sum()
#lazy print
print(passengers_per_day)  
avg_fare = df.fare_amount.mean()
#lazy print
print(f"Average fare: {avg_fare}")  
#Evaluate task graph including lazy prints
pd.flush()  
\end{lstlisting}
% \end{mypython}

Listing \ref{lazy_print_ex} presents an example with multiple print statements, and the equivalent task graph is shown in Figure \ref{fig:lazy_print_ex_img}. We first override the built-in print method with LaFP's lazy print method. This can be done by adding one of the statements below.

\begin{center}
\begin{verbatim}
from lazyfatpandas.func import print 
print = pd.lazyPrint
\end{verbatim}
\end{center}
\label{print_override}


When LaFP's lazy print is called, all the lazy DataFrames used in the print statement are identified. These lazy DataFrames must be computed before the lazy print is executed. The node representing the print operation is added to the task graph, with the lazy DataFrames as the source nodes. A dependency edge is added to the previous print operation (if any) to maintain the correct print order.




\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/lazy_print_ex_img.pdf}
        \caption{LaFP task graph executed during the call to flush in Listing \ref{lazy_print_ex}}
        \label{fig:lazy_print_ex_img}
\end{figure}

At the end of the program, \texttt{pd.flush} is called, which internally invokes \texttt{compute} on the last print node, forcing the computation of the task graph. The print statements are processed in the correct order due to the dependency edges between print nodes. The statements \texttt{print = pd.lazyPrint} and \texttt{pd.flush()} are automatically inserted in the source program by \SCIRPy, fully automating the process.


\subsection*{Lazy Printing with f-strings}
As mentioned earlier, we need to detect the lazy DataFrames used in a print statement because these DataFrames must be computed before the lazy print can be processed. The problem arises when a DataFrame is used in Python's formatted strings (f-strings), as the DataFrame value is needed to construct the string. To build the string while avoiding computation, we use the unique ID of the task graph node representing the DataFrame and an escape sequence to mark the unique ID. When the constructed string is passed to the lazy print method, we check for the escape sequence to identify the unique ID of the task graph node. This node must be computed when the lazy print is processed at the end of the program. For example, in Line 12 of Listing \ref{lazy_print_ex}, the DataFrame \texttt{avg\_fare} is used in an f-string. The string that will be constructed is \texttt{"Average fare: \$\_\#UID\$\_\#"}. When lazy prints are processed, \texttt{"\$\_\#UID\$\_\#"} is replaced by the value of the computed DataFrame.

\subsection{Forced Computation for Non-Lazy Function Call}\label{sec:force_compute}
Dask and other lazy frameworks do not natively support non-lazy third-party modules that expect an evaluated Pandas DataFrame. The users have to manually force a computation before Dataframe can be passed to these API calls. LaFP also faced the same problem. Further, as these modules, such as \texttt{matplotlib}, are a black box to LaFP, delaying the DataFrame computation, beyond the API call is infeasible. Therefore, to improve interactivity, when such non-lazy modules are called, LaFP forces computation and computed Dataframe is passed to the API call.


% \begin{mypython}[caption={Program with external module}, label=force_compute_ex]
\begin{lstlisting}[language=Python, caption=Program with external module, label=force_compute_ex]
import lazyfatpandas.pandas as pd
#external module
import matplotlib.pyplot as plt  
#override built-in print with lazy print
print = pd.lazyPrint  
df = pd.read_csv("data.csv", parse_dates=["pickup_datetime"])
print(df.head())  # lazy print
df["day"] = df.pickup_datetime.dt.dayofweek
passengers_per_day = df.groupby(["day"])["passenger_count"].sum()
#pending lazy prints evaluated when 
#passengers_per_day is computed and passed to plt.plot
plt.plot(passengers_per_day.compute())
plt.savefig("fig.png")
avg_fare = df.fare_amount.mean()
#lazy print
print(f"Average fare: {avg_fare}")  
#evaluate remaining lazy prints (line 17)
pd.flush()  
\end{lstlisting}

Further, since external modules like \texttt{matplotlib.pyplot} can generate output, this can conflict with lazy printing by changing the output order. To solve this issue, pending print operations are processed when a DataFrame is forced to compute, maintaining the correct output order.

Program in Listing \ref{force_compute_ex} demonstrates forced computation. \SCIRPy\ keeps track of all the external non-lazy modules imported during program rewriting, like \texttt{plt}, the alias of \texttt{matplotlib.pyplot}. \SCIRPy\ checks whether a DataFrame is passed as an argument when these modules are used. If found, the statement is rewritten, and \texttt{compute} is called, like in Line 12 of the example program. 




% Third rule (return type) has not been implemented yet

\begin{lstlisting}[language=Python, caption=Cases where new DataFrame variables are created, label=force_compute_ex1]
# df is the source DataFrame
df1 = pd.read_csv(data.csv) 
# operations on a DataFrame yield a new DataFrame
df2 = df.head()             
# operations on a DataFrame yield a new DataFrame
df3 = df[df.column > 0]     
# return type is a DataFrame
df4 = func(...)             
\end{lstlisting}



\begin{figure*}
    \begin{minipage}{0.4\textwidth}
        \centerline{\includegraphics[width=.93\textwidth]{figures/force_compute_img1.pdf}}
        \caption{Task graph executed in Line 13 of Listing \ref{force_compute_ex}}
        \label{fig:force_compute_img1}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.4\textwidth}
        \centerline{\includegraphics[width=.93\textwidth]{figures/force_compute_img2.pdf}}
        \caption{Task graph executed in Line 19 of Listing \ref{force_compute_ex}}
        \label{fig:force_compute_img2}
    \end{minipage}
\end{figure*}


% \subsection*{Forced Computation for Non-Lazy Function Calls}


% \vspace{.15cm}

In Line 12 of Listing \ref{force_compute_ex}, when \texttt{passengers\_per\_day} is computed, the task graph shown in Figure \ref{fig:force_compute_img1} is executed. The lazy print in Line 7 is processed, and the result of the node \texttt{sum} (value of \texttt{passengers\_per\_day}) is returned and passed to \texttt{plt.plot}, generating a plot image. Finally, when \texttt{pd.flush} is called in Line 18, the print in Line 16 is processed, and the task graph shown in Figure \ref{fig:force_compute_img2} is executed.

\vspace{.15cm}

Notice that the sub-tree rooted at node \texttt{set\_item day} is recomputed when \texttt{pd.flush} is called. This is because, in Line 13, when \texttt{passengers\_per\_day} is computed, information related to the future usage of the DataFrames in the rest of the program is unavailable. This issue and its solution are further discussed in Section \ref{sec:persist_live_df}.

\subsection*{Inferring DataFrames in the Program}
To invoke \texttt{compute} on a DataFrame, we need to figure out which variables are DataFrame variables. To infer the DataFrame variables, we use three rules:
\begin{enumerate}
    \item First, the source DataFrame is created using \texttt{read\_csv}, \\ \texttt{read\_parquet} or similar APIs.
    \item Second, any operation on a DataFrame except in-place operations returns a DataFrame or Series. 
    \item Third, the value returned from a function is a DataFrame. 
\end{enumerate}
 \SCIRPy\ uses these rules to keep track of DataFrames that are created or updated in the program.

 
\subsection{Common Computation Reuse}
Since Dask employs lazy evaluation, the result of any operation on a Dask collection is a lazy Dask collection. To force the computation, we must invoke \texttt{dask-compute}\footnote{Dask-compute refers to the compute operation on a Dask collection.}. \texttt{Dask-compute} returns the in-memory equivalent Pandas or NumPy object, but intermediate computations (the results of intermediate nodes) are not retained. 

\vspace{.15cm}

For example, in Figure \ref{fig:task_graph_eval_img}, the nodes \texttt{get\_item [filter]} and \texttt{mean} are printed. If we call \texttt{dask-compute} on the lazy Dask collection stored in the \texttt{result} field of the \texttt{get\_item [filter]} node, the dataset is read, and the filter operation is performed. Later, when \texttt{dask-compute} is called on the \texttt{result} of \texttt{mean}, the dataset is read again, the filter operation is repeated, and the mean of \texttt{passenger\_count} is calculated. These operations, such as reading the dataset and applying the filter, are repeated because \texttt{dask-compute} does not maintain intermediate computations.

\vspace{.15cm}

In order to avoid recomputing same operations again, we use \texttt{dask-persist}\footnote{Dask-persist refers to the persist operation on a Dask collection.}. When \texttt{dask-persist} is called on a Dask collection, the computation is forced, and a new Dask collection backed by in-memory data is returned. This means that computations up to that point are performed and stored in memory. Thus, when a node is needed multiple times, we use \texttt{dask-persist} to save the node's memory-backed \texttt{result} and avoid recomputing it when needed again. 




In the previous example, the \texttt{read\_csv} and \texttt{get\_item [filter]} nodes are needed multiple times (in-degree greater than one). Therefore, when these nodes are executed, we invoke \texttt{dask-persist} on the resulting lazy Dask collection and store the in-memory backed Dask collection in the \texttt{result} field. Finally, when \texttt{dask-compute} is called on \texttt{get\_item [filter]} and \texttt{mean} for printing, Dask uses the persisted data for computation, preventing the recomputation of sub-expressions.






 

